Explicit block encodings of boundary value problems for many-body elliptic operators

Simulation of physical systems is one of the most promising use cases of future digital quantum computers. In this work we systematically analyze the quantum circuit complexities of block encoding the discretized elliptic operators that arise extensively in numerical simulations for partial differential equations, including high-dimensional instances for many-body simulations. When restricted to rectangular domains with separable boundary conditions, we provide explicit circuits to block encode the many-body Laplacian with separable periodic, Dirichlet, Neumann, and Robin boundary conditions, using standard discretization techniques from low-order finite difference methods. To obtain high-precision, we introduce a scheme based on periodic extensions to solve Dirichlet and Neumann boundary value problems using a high-order finite difference method, with only a constant increase in total circuit depth and subnormalization factor. We then present a scheme to implement block encodings of differential operators acting on more arbitrary domains, inspired by Cartesian immersed boundary methods. We then block encode the many-body convective operator, which describes interacting particles experiencing a force generated by a pair-wise potential given as an inverse power law of the interparticle distance. This work provides concrete recipes that are readily translated into quantum circuits, with depth logarithmic in the total Hilbert space dimension, that block encode operators arising broadly in applications involving the quantum simulation of quantum and classical many-body mechanics.

==> SuccessProb.tex <==
In constructing the system of equations resulting from discretization of the affiliated differential operators, one must encode in the right hand side $\mathbf{b}$ the initial data from the boundary conditions, and additionally place a $1$ on the diagonal of the matrix corresponding to the node where the boundary data is known. 

On the quantum computer, the workflow begins by preparing a quantum state $\ket{b}$ on the system register that corresponds to the right hand side of the differential equaiton. For the Dirichlet problem, one might have
\begin{equation}
\begin{aligned}
    L[u] &= 0\\
    u(0) &= 0\\
    u(1) &= 1,
\end{aligned}
\end{equation} 
where $\ket{b}$ is simply the basis vector $\ket{N-1}$ after appropriate normalization. Then, the next step is to prepare the block-encoding and apply it to $\ket{b}$. Now we seek to obtain a bound on the success probability in terms of $N$. The first step is the application of $A$, the matrix representation of the problem, onto $\ket{b}$. The success probability of this first step is crucial to the efficiency of the algorithm. 

We seek to obtain a lower bound to
\begin{equation}
    ||\mathcal{L}\ket{b}||^2 = |\bra{b}\mathcal{L}^\dagger \mathcal{L}\ket{b}|,
    \label{eq: success prob eqn}
\end{equation}
which we then divide by $d$ times the one dimensional subnormalization factor
\begin{equation}
    \alpha_d = d\sum_{j=-a}^a|r_j|
\end{equation}
We will have $d^2$ terms in \eqref{eq: success prob eqn}. $d$ of these terms are given by
\begin{equation}
    L_0^\dagger L_0 \otimes I^{d-1}, I\otimes L_1^\dagger L_1 \otimes I^{d-2}, \ldots, I^{\otimes d-1}\otimes L_d^\dagger L_d.
\end{equation}
Since each of these operators are $1$-local it suffices to consider only the the action of $L_j^\dagger L_j$ on the subspace corresponding to the $d$th dimension, as the other terms in the tensor product contribute a multiplicative factor of $1$.

We have for the $j$th term of this form
\begin{align*}
    \frac{1}{N_j}\sum_{k,l \in B_j}\bra{k}L_j^\dagger L_j\ket{l}\ket{l}\\
\end{align*}
but since each $k \in A_j$ is by definition either on the boundary or interior of the boundary region, $L$ is diagonal in that region so that $L\ket{k} = -r_0\ket{k}$, so this allows us to obtain a bound
\begin{align*}
    \vert{\frac{1}{N_j}\sum_{k,l\in A_j} \bra{k}L^\dagger L \ket{l}\vert} \geq \vert\sum_{i = 1}^{N_j}\frac{r_0^2}{N_j}\vert =r_0^2
\end{align*}
which is a lower bound that is independent of $N_j$. Doing this for each of these $d$-terms, we find a lower bound for the norm of these one-local terms as
\begin{equation}
    dr_0^2
\end{equation}
The rest of the terms are 2-local with $L_j$ acting on one site $L_k^\dagger$ acting on another site. If both $L_k$ and $L_j^\dagger$ are acting on each of their respective boundary registers, of which there are also $d$ of these terms $\mathcal{D}_k\ket{0}$ and $\mathcal{D}_j\ket{0}$ then the contribution will be of the same order given above, i.e.
\begin{equation}
    dr_0^2.
\end{equation}
If only one of $L_j$ or $L_k^\dagger$ is acting on it's respective boundary ket, and the other is operating on another boundary register $\mathcal{D}_i\ket{0}$ then we expect to see a contribution of the order $\frac{1}{N_i}$, of which there are $d$ of. This gives an additional contribution that is 
\begin{equation}
    O\left(d\sum_{j=0}^{d-1}\frac{1}{N_j}\right) 
\end{equation}
Finally, if neither $L_j$ nor $L_k^\dagger$ is acting on their respective registers which there are $2(d^2-d)$ terms like this, we can expect an additional contribution that is $O(1/(N_l N_i))$, which gives a contribution that is
\begin{equation}
    O\left(2d(d-1)\sum_{i,j=0}^{d-1}\frac{1}{N_i N_j}\right).
\end{equation}
Therefore the total success probability will be the sum of each of these terms
\begin{equation}
    P_{\text{succ}} = \frac{1}{d^2\alpha^2}\left(2dr_0^2 + d\sum_{j=0}^{d-1}\frac{1}{N_j} + 2d(d-1)\sum_{i,j=0}^{d-1}\frac{1}{N_i N_j}\right).
\end{equation}
We can therefore obtain a lower bound to the success probability as 
\begin{equation}
   P_{\text{succ}} > \frac{2dr_0^2}{d^2 \alpha} > \frac{6r_0^2}{2d\pi^2} > \frac{6 \left(\frac{2\pi ^2}{3}\right)^2}{2d\pi^2} = \frac{4 \pi ^2}{3 d}
\end{equation}
where the second to last and last inequalities are direct applications of the bound given in \eqref{eq: alpha upper bound}. Which is constant in $N$ and inverse linear in $d$. Knowing the particular boundary geometry allows one to obtain tighter bounds.


\textbf{d = 1}
The success probability can be estimated by computing $||A\ket{b}||$. Let's consider an example in one spatial dimension for one particle, where the boundary data specifies that $u(0) = 0$ and $u(1) = 1$. Here, the system of equations we form has the structure
\begin{equation}
    \begin{bmatrix}
        -2 & 0 & 0&0& \cdots & 0\\
        1 & -2 & 1 &0&\cdots & 0\\
        0 & 1 & -2 &1& \cdots & 0\\
        \vdots &\vdots &\ddots & \ddots &\ddots & \vdots\\
        0 & 0 & \ldots& 1 & -2 & 1\\
        0 & 0 & \ldots& 0 & 0 & -2
    \end{bmatrix}
    \begin{bmatrix}
        u(x_0)\\
        u(x_1)\\
        u(x_2)\\
        \vdots \\
        u(x_{N-2})\\
        u(x_{N-1})
    \end{bmatrix}
    =
    \begin{bmatrix}
        0\\
        0\\
        0\\
        \vdots \\
        0\\
        -2
    \end{bmatrix}.
\end{equation}


Presented using the shift operators, this equation becomes
\begin{equation}
    \left[-2I + \frac{1}{2}\left(S^1 + S^1_{N-2,N-1}\right) + \frac{1}{2}\left(S^{-1} + S^{-1}_{0,1}\right)\right]\ket{u(x)} = -2 \ket{N-1}
    \label{eq:1d alg equation}
\end{equation}
We divide the matrix on the left hand side by the LCU subnormalization factor 
\begin{equation}
    \alpha = \sum_{i=1}^5 |c_i| = 4.
\end{equation}
Furthermore, we require the right hand side also be normalized, so we replace $-2\ket{N-1}$ with $\ket{N-1}$.

For the 1D case, we compute 
\begin{equation}
    ||L\ket{N-1}||^2 = |\bra{N-1}L^\dagger L \ket{N-1}| = 5
\end{equation}
so that the success probability 
\begin{equation}
    P_{\text{succ}} = \frac{1}{\alpha^2}||L\ket{N-1}||^2
\end{equation}
becomes
\begin{equation}
   \frac{5}{16} \sim .3125
   \label{eq:1d success prob}
\end{equation}
which is a constant.


\textbf{d=2}:

In $2$ dimensions, the boundary condition becomes
\begin{equation}
    u(x=L,y) = 1
\end{equation}
which, upon discretization corresponds to the right hand side vector becoming
\begin{equation}
    \ket{b} = \ket{N-1}\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}
\end{equation}
and the matrix representation of the operator also becomes
\begin{equation}
    \frac{1}{2\alpha}\left(L\otimes I + I \otimes L\right).
\end{equation}
As above, we wish to bound
\begin{equation}
    ||\left(L\otimes I + I \otimes L\right)\ket{b}||^2 = |\bra{b}\left(L\otimes I + I \otimes L\right)^2\ket{b}|,
\end{equation}
after which we divide by $10$ in order to obtain the success probability with an LCU block-encoding. An equivalent expression for the norm is given by 
\begin{equation}
    |\bra{b}\left(L^\dagger L \otimes I + I \otimes L^\dagger L + L^\dagger \otimes L + L\otimes L^\dagger\right )\ket{b}|
\end{equation}

Taking this term by term, the first term 
\begin{align*}
    &\bra{b}L^\dagger L \otimes I\ket{b} = \bra{N-1}\frac{1}{N}\sum_{i=0}^{N-1}\bra{i}(L^\dagger L\otimes I)\ket{N-1}\sum_{j=0}^{N-1}\ket{j}\\
    &=\frac{1}{N}\left(\bra{N-1}L^\dagger L\ket{N-1}\times \sum_{i,j}\bra{i}\ket{j}\right)\\
    &=\frac{1}{N}\left(5\times \sum_{i,j}\bra{i}\ket{j}\right)\\
    &=\frac{5}{N}\left(\times N\right)\\
    &=5,
\end{align*}

the second term
\begin{align*}
    &\bra{b}I \otimes L^\dagger L \ket{b} = \bra{N-1}\frac{1}{N}\sum_{i=0}^{N-1}\bra{i}(I\otimes L^2)\ket{N-1}\sum_{j=0}^{N-1}\ket{j}\\
    &=\frac{1}{N}\sum_{i,j=0}^{N-1}(\bra{N-1}\ket{N-1}\bra{i}L^\dagger L\ket{j})\\
    &=\frac{1}{N}\sum_{i,j=0}^{N-1}(\bra{i}L^\dagger L \ket{j})\\
    &= \frac{1}{N}\times8\\
    &=\frac{8}{N},
\end{align*}

and the third term
\begin{align*}
    &\bra{b}L^\dagger\otimes L\ket{b} = \frac{1}{N}\sum_{i,j=0}^{N-1}(\bra{N-1}L^\dagger \ket{N-1} \bra{i}L\ket{j})\\
    &=\frac{\bra{N-1}L^\dagger\ket{N-1}}{N}\sum_{i,j=0}^{N-1}(\bra{i}L\ket{j})\\
    &=\frac{-2}{N}\sum_{i,j=0}^{N-1}\bra{i}L^\dagger\ket{j}\\
    &=\frac{8}{N}.
\end{align*}
Here we used the facts that $\bra{N-1}L^\dagger \ket{N-1} = -2$ and $\sum_{ij}L_{ij} = -4$.

The fourth term is similar,
\begin{align*}
    &\bra{b}L\otimes L^\dagger\ket{b} = \frac{1}{N}\sum_{i,j=0}^{N-1}(\bra{N-1}L \ket{N-1} \bra{i}L^\dagger\ket{j})\\
    &=\frac{\bra{N-1}L\ket{N-1}}{N}\sum_{i,j=0}^{N-1}(\bra{i}L^\dagger\ket{j})\\
    &=\frac{-2}{N}\sum_{i,j=0}^{N-1}(\bra{i}L\ket{j})\\
    &=\frac{8}{N}.
\end{align*}
Adding up each of the individual contributions, we obtain our estimate to the success probability as 
\begin{equation}
    5 + \frac{16}{N} + \frac{8}{N} = 5+\frac{24}{N}
\end{equation}
which, is again a constant. The LCU subnormalization  contributes a factor of $\frac{1}{(2\alpha)^2}$, to the success probability giving 
\begin{equation}
    P_{\text{succ}} = \frac{5 + \frac{33}{2N}}{64} \sim .078 \text{ as } N\rightarrow \infty
\end{equation}

We learned that the overlaps for each of these terms respectively satisfy
\begin{align*}
    L^\dagger L \otimes I &\rightarrow 5\\
    I\otimes L^\dagger L &\rightarrow \frac{8}{N}\\
    L^\dagger\otimes L \text{ or h.c. } &\rightarrow \frac{8}{N}
\end{align*}


\textbf{d=3}
We work through the case where $d=3$, this time we have
\begin{equation}
    \mathcal{L} = L\otimes I \otimes I + I\otimes L \otimes I + I\otimes I \otimes L
\end{equation}
and
\begin{equation}
    \ket{b} = \ket{N-1}\otimes \frac{1}{N}\sum_{i,j}\ket{i}\otimes\ket{j}.
\end{equation}

We have terms of the form $L^\dagger L\otimes I \otimes I$ and $I\otimes L^\dagger L \otimes I$, in addition, we have terms of the form 
$L^\dagger \otimes L \otimes I$ + h.c. and $I\otimes L^\dagger \otimes L$ + h.c.

We can use the results from the previous table, to get 
\begin{equation}
    \bra{b} L^\dagger L \otimes I \otimes I \ket{b} = 5
\end{equation}
and
\begin{equation}
    \bra{b}(I\otimes L^\dagger L \otimes I + I\otimes I \otimes L^\dagger L)\ket{b} = \frac{16}{N}
\end{equation}
and
\begin{align}
    &\bra{b}(L^\dagger \otimes I \otimes L + L^\dagger\otimes L \otimes I + h.c.)\ket{b} \nonumber\\
    &=\frac{8}{N} + \frac{8}{N} +\frac{8}{N} + \frac{8}{N} \nonumber\\
    &= \frac{32}{N}.
\end{align}

The final terms are the ones where we have two Laplacian operators acting on the uniform superposition sites, and none acting on the register containing $\ket{N-1}$
\begin{align}
&\bra{b}(I\otimes L \otimes L^\dagger + I\otimes L^\dagger \otimes L)\ket{b}.
\end{align}

It suffices to consider 
\begin{align*}
    &\frac{1}{N^2}\sum_{ijkl}\bra{i}\bra{j}(L^\dagger \otimes L)\ket{k}\ket{l}\\
    &=\frac{1}{N^2}\sum_{ijkl}\bra{i}L^\dagger \ket{k} \bra{j}L\ket{l}\\
    &=\frac{1}{N^2}\sum_{ik}\bra{i}L^\dagger \ket{k}\sum_{jl} \bra{j}L\ket{l}\\
    &=\frac{1}{N^2}(-4)(-4)\\
    &=\frac{16}{N^2}
\end{align*}
of which there are two of them, so we obtain
\begin{equation}
    \bra{b}(I\otimes L \otimes L^\dagger + I\otimes L^\dagger \otimes L)\ket{b} = \frac{32}{N^2}
\end{equation}

Now, we add up all the contributions, and we obtain
\begin{equation}
   ||\mathcal{L}\ket{b}||^2 =  5 + \frac{48}{N} + \frac{32}{N^2}.
\end{equation}
We then divide through by the subnormalization factor $\frac{1}{(3\alpha)^2} = \frac{1}{144}$ to obtain 
\begin{equation}
    P_{\text{succ}} = \frac{1}{144}( 5 + \frac{33}{N} + \frac{32}{N^2})
\end{equation}
which in the large $N$ limit gives a success probability that is 
\begin{equation}
    P_{\text{succ}} = \frac{5}{144} \sim .0347
\end{equation}

\subsection{Arbitrary dimension}
Here we consider the general case of computing 
\begin{equation}
    |\bra{b}\mathcal{L}\ket{b}|^2
\end{equation}
for
\begin{equation}
    \mathcal{L} = \underset{d}{\underbrace{L\otimes \underset{d-1}{\underbrace{I \otimes I \otimes \cdots \otimes I}} + \cdots +I\otimes I \otimes \cdots \otimes L}}
\end{equation}
and
\begin{equation}
    \ket{b} = \frac{1}{\sqrt{N^{d-1}}} \ket{N-1}\otimes \sum_{i_1,i_2,\ldots,i_{d-1}}\ket{i_1}\ket{i_2}\cdots\ket{i_{d-1}}.
\end{equation}

We will have one term of the form $L^\dagger L$ acting on $\ket{N-1}$, we will have (d-1) terms as $L^\dagger L$ acting on a uniform superposition state, and $2\binom{d}{2}$ terms with action an operator $L$ or $L^\dagger$ acting on two sites. Of the ``weight two" terms, we have $2d$ terms where either $L$ or $L^\dagger$ is acting on the $\ket{N-1}$ state with an $L$ or $L^\dagger$ acting anywhere else and we have $2d^2 - 2d$ terms where both sites are acting on the uniform superposition registers.

The first term gives
\begin{equation}
    \bra{N-1}L^\dagger L\ket{N-1} = 5
\end{equation}
the second kinds of terms, i.e. the weight 1, no support on 0th-direction register, of which there are $d-1$ of, each contribute $\frac{8}{N}$ in total contribute:
\begin{equation}
 \frac{8(d-1)}{N}
\end{equation}
the third kinds of term where there is only $L$ or $L^\dagger$ acting on the 0th direction register and a random $L$ elsewhere, there are $2d$ of those, each contribute $\frac{8}{N}$ in total:
\begin{equation}
    \frac{16d}{N}
\end{equation}
the fourth kinds of terms where neither $L$ nor $L^\dagger$ has support on the $\ket{N-1}$ state, each contribute $16/N^2$ of which there are $2(d^2-d)$ of, gives
\begin{equation}
    \frac{32(d^2-d)}{N^2}
\end{equation}

Adding these up, we find
\begin{equation}
    |\bra{b}\mathcal{L}\ket{b}|^2 = 5 +  \frac{8(d-1) + 16d}{N} + \frac{32(d^2-d)}{N^2},
\end{equation}
so that the success probability, which is multiplied by $\frac{1}{(4d)^2}$ becomes
\begin{equation}
    P_{\text{succ}} = |\bra{b}\mathcal{L}\ket{b}|^2 =\frac{5 +  \frac{8(d-1) + 16d}{N} + \frac{32(d^2-d)}{N^2}}{d^2}
\end{equation}
whenever $d>2$.

In the large $d$ limit, we obtain
\begin{equation}
    P_{\text{large dim}} = \frac{33}{16N^2}
\end{equation}
and in the large $N$ limit, we obtain
\begin{equation}
    P_{\text{large grid}} = \frac{5}{16d^2}
\end{equation}
and in the $d = O(N)$ limit, we obtain
\begin{equation}
    p_{d\sim N} = \frac{62N - 41}{16N^3} = O(1/N^2)
\end{equation}
For a large grid where $N \gg d$, we see that the expected scaling for the success probability is $O(1/d^2)$ with the preconstant $5/16 = 5/\alpha^2$.


==> commands.tex <==

% Quantum Computing commands
\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\QFT}{\mathrm{QFT}}
% \newcommand{\gcd}{\mathrm{gcd}}
\newcommand{\Hrm}{\mathrm{H}}
\newcommand{\expec}[1]{\langle #1 \rangle}
\newcommand{\BE}{\operatorname{BE}} % block encoding
\newcommand{\comp}{\mathfrak{comp}}
\newcommand{\dom}{\mathfrak{dom}}


% Include in preamble of most files
\iffalse
\usepackage{amsmath, amssymb, amsthm, thmtools, mathtools}%solution style
\usepackage{cancel,enumitem, float}
\usepackage{fancyhdr,import, graphicx, color}
\usepackage{todonotes} % [disable] option is available
\usepackage{hyperref}
\usepackage{siunitx}
\usepackage{braket}
\hypersetup{
	colorlinks = true,
	citecolor = red,
	linkcolor = blue
}

% Figure and Table Templates
\begin{figure}[H]
	\centering
	\input{}
	\caption{}
	\label{fig:}
\end{figure}
\fi

\usepackage{bm}
\usepackage{mathrsfs}
% \usepackage{sectsty}


% Custom Colours
\usepackage{xcolor}
\definecolor{berkeley-blue}{HTML}{003262}
\definecolor{berkeley-gold}{HTML}{C4820F}
% \sectionfont{\color{berkeley-blue}}

% Multi Column
\usepackage{multicol}
\setlength{\columnseprule}{1pt} %Separator ruler width
\def\columnseprulecolor{\color{berkeley-blue}} %Separator ruler colour

%------------------- Theorem Styles ------------------------------------




%-------------------Custom Commands------------------------------------
\newcommand{\CPn}{\bbC\bbP^n}
\newcommand{\RPn}{\bbR\bbP^n}
\newcommand{\Bbar}{\bar{\mathbb{B}}}


\newcommand{\parder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\bracfrac}[2]{\left(\frac{#1}{#2}\right)}


% Custom Operators
% \newcommand{\tr}{\operatorname{tr}}
% \newcommand{\Tr}{\operatorname{Tr}}
% \newcommand{\grad}{\operatorname{grad}}
% \newcommand{\Grad}{\operatorname{Grad}}
% \newcommand{\divg}{\operatorname{div}}
%\newcommand{\divb}{\boldsymbol{\operatorname{div}}}
% \newcommand{\curl}{\operatorname{curl}}

\newcommand{\vol}{\text{vol}}

\newcommand{\HRule}{\rule{\linewidth}{0.5mm}} % Command to make the lines in the title page

\newcommand{\etal}{\emph{et al.} }
\newcommand{\noi}{\noindent}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

\newcommand\encircle[1]{%
	\tikz[baseline=(X.base)] 
	\node (X) [draw, shape=circle, inner sep=0] {\strut #1};}

%---------------------- Letters and Such -------------------------------

% Scripted Letters
\newcommand{\scrB}{\mathscr{B}}
\newcommand{\scrI}{\mathscr{I}}
\newcommand{\scrS}{\mathscr{S}}

% Mathbold symbols
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbH}{\mathbb{H}}

% Caligraphy Symbols
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%% Bold Symbols

% Alphabet
\newcommand{\abm}{\bm{a}}
\newcommand{\bbm}{\bm{b}}
\newcommand{\cbm}{\bm{c}}
\newcommand{\dbm}{\bm{d}}
\newcommand{\ebm}{\bm{e}}
\newcommand{\fbm}{\bm{f}}
\newcommand{\gbm}{\bm{g}}
\newcommand{\hbm}{\bm{h}}
\newcommand{\ibm}{\bm{i}}
\newcommand{\jbm}{\bm{j}}
\newcommand{\kbm}{\bm{k}}
\newcommand{\lbm}{\bm{l}}
\newcommand{\mbm}{\bm{m}}
\newcommand{\nbm}{\bm{n}}
\newcommand{\obm}{\bm{o}}
\newcommand{\pbm}{\bm{p}}
\newcommand{\qbm}{\bm{q}}
\newcommand{\rbm}{\bm{r}}
\newcommand{\sbm}{\bm{s}}
\newcommand{\tbm}{\bm{t}}
\newcommand{\ubm}{\bm{u}}
\newcommand{\vbm}{\bm{v}}
\newcommand{\wbm}{\bm{w}}
\newcommand{\xbm}{\bm{x}}
\newcommand{\ybm}{\bm{y}}
\newcommand{\zbm}{\bm{z}}
\newcommand{\Abm}{\bm{A}}
\newcommand{\Bbm}{\bm{B}}
\newcommand{\Cbm}{\bm{C}}
\newcommand{\Dbm}{\bm{D}}
\newcommand{\Ebm}{\bm{E}}
\newcommand{\Fbm}{\bm{F}}
\newcommand{\Gbm}{\bm{G}}
\newcommand{\Hbm}{\bm{H}}
\newcommand{\Ibm}{\bm{I}}
\newcommand{\Jbm}{\bm{J}}
\newcommand{\Kbm}{\bm{K}}
\newcommand{\Lbm}{\bm{L}}
\newcommand{\Mbm}{\bm{M}}
\newcommand{\Nbm}{\bm{N}}
\newcommand{\Obm}{\bm{O}}
\newcommand{\Pbm}{\bm{P}}
\newcommand{\Qbm}{\bm{Q}}
\newcommand{\Rbm}{\bm{R}}
\newcommand{\Sbm}{\bm{S}}
\newcommand{\Tbm}{\bm{T}}
\newcommand{\Ubm}{\bm{U}}
\newcommand{\Vbm}{\bm{V}}
\newcommand{\Wbm}{\bm{W}}
\newcommand{\Xbm}{\bm{X}}
\newcommand{\Ybm}{\bm{Y}}
\newcommand{\Zbm}{\bm{Z}}

% Greek
\newcommand{\sigmabm}{\bm{\sigma}}

% ------------------------- From Kranthi -----------------------------------

% KM CBE256 HW1
\newcommand{\diver}{\text{div}}
\newcommand{\gradi}{\text{grad}}
\newcommand{\curli}{\text{curl}}


%% Lower Case bold letters                                  \mathbf{} 
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
%\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
%\newcommand{\ob}{\mathbf{o}}
% \newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
% \newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}


%% Upper Case bold letters                                  \mathbf{} 
\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

%% Caligraphy  Math symbols 			\mathcal{}

\newcommand{\Bs}{{\mathscr B}}
\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Fc}{{\mathcal F}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Jc}{{\mathcal J}}
\newcommand{\Kc}{{\mathcal K}}
\newcommand{\Lc}{{\mathcal L}}
\newcommand{\Mc}{{\mathcal M}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Qc}{{\mathcal Q}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Wc}{{\mathcal W}}
\newcommand{\Xc}{{\mathcal X}}
\newcommand{\Yc}{{\mathcal Y}}
\newcommand{\Zc}{{\mathcal Z}}

\newcommand{\zerob}{{\boldsymbol{0}}}

% Greek
\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\epsb}{\boldsymbol{\epsilon}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\Phib}{\boldsymbol{\Phi}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\nablab}{\boldsymbol{\nabla}}
\newcommand{\gammab}{\bm{\gamma}}
\newcommand{\Gammab}{\mathbf{\Gamma}}
\newcommand{\dm}{\mathrm{d}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\chib}{\bm{\chi}}
\newcommand{\omegab}{\boldsymbol{\omega}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}


\newcommand{\dt}{\Delta t}
%\newcommand{\sB}{{\mathscr B}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\Pp}{{\partial \cP}}



